RoboTwin: Dual-Arm Robot Benchmark with Generative Digital Twins

In the rapidly advancing field of robotics, dual-arm coordination and complex object manipulation are essential capabilities for developing advanced autonomous systems. However, the scarcity of diverse, high-quality demonstration data and real-world-aligned evaluation benchmarks severely limits such development. To address this, we introduce RoboTwin, a generative digital twin framework that uses 3D generative foundation models and large language models to produce diverse expert datasets and provide a real-world-aligned evaluation platform for dual-arm robotic tasks. Specifically, RoboTwin creates varied digital twins of objects from single 2D images, generating realistic and interactive scenarios. It also introduces a spatial relation-aware code generation framework that combines object annotations with large language models to break down tasks, determine spatial constraints, and generate precise robotic movement code. Our framework offers a comprehensive benchmark with both simulated and real-world data, enabling standardized evaluation and better alignment between simulated training and real-world performance. We validated our approach using the open-source COBOT Magic Robot platform. Policies pre-trained on RoboTwin-generated data and fine-tuned with limited real-world samples demonstrate significant potential for enhancing dual-arm robotic manipulation systems by improving success rates by over 70% for single-arm tasks and over 40% for dual-arm tasks compared to models trained solely on real-world data.

==> sec/3_preliminary.tex <==
\section{Preliminary}
\subsection{Diffusion Model as Policy}
We formulate the dexterous manipulation planning problem within the Markov Decision Process (MDP) framework~\cite{puterman1994markov}, defined as $\mathcal{M}=(\mathcal{S}, \mathcal{A}, \mathcal{T}, \mathcal{R}, \gamma)$. The objective is to find an optimal action sequence $\ba_{0:T}^*$ that maximizes the expected cumulative rewards over horizon $T$:
\vspace{-5pt}
\begin{equation}
\ba_{0:T}^*=\underset{\ba_{0:T}}{\arg \max } \mathcal{J}(\bs_0, \ba_{0:T})=\underset{\ba_{0:T}}{\arg \max } \sum_{t=0}^T \gamma^t R(\bs_t, \ba_t),
\vspace{-2pt}
\end{equation}
where state transitions follow $\bs_{t+1}=\mathcal{T}(\bs_t, \ba_t)$.

Following~\cite{diffuser,decisiondiffuser}, we leverage diffusion models to address this planning problem by treating state or action trajectories $\btau$ as sequential data. The diffusion process gradually adds Gaussian noise to the data over $N$ steps, while the reverse process learns to denoise trajectories through conditional probability $p_\theta(\btau^{i-1} \mid \btau^i)$. The model is trained to maximize the likelihood:
\vspace{-5pt}
\begin{equation}
p_\theta\left(\btau^0\right)=\int p\left(\btau^N\right) \prod_{i=1}^N p_\theta\left(\btau^{i-1} \mid \btau^i\right) \mathrm{d} \btau^{1: N},
\vspace{-2pt}
\end{equation}
with the optimization objective inspired by evidence lower bound (ELBO), where $p\left(\btau^N\right)$ is a standard normal distribution and $\btau^{0}$ denotes original sequence data:
\begin{equation}
% \small
\theta^*=\arg \min _\theta-\mathbb{E}_{\btau^0}\left[\log p_\theta\left(\btau^0\right)\right],
\label{eq:theta_optim}
\vspace{-3pt}
\end{equation}

For practical implementation, we adopt the simplified surrogate loss~\cite{ddpm} that focuses on predicting the noise term:
\vspace{-3pt}
\begin{equation}
\mathcal{L}_{\text{denoise}}(\theta) = \mathbb{E}_{i, \btau^{0} \sim q, \epsilon \sim \mathcal{N}}[||\epsilon - \epsilon_{\theta}(\btau^i, i)||^{2}].
\label{eq:loss_uncond}
% \vspace{-2pt}
\end{equation}

\subsection{Classifier-free Conditional Policy}
To generate high-reward trajectories, classifier-free guidance~\cite{diffusion_beatgan} has been transferred from image to trajectory generation~\cite{decisiondiffuser}. This approach incorporates guidance signals $\boldsymbol{y}(\btau)$ that emphasize desired trajectory characteristics. The noise prediction is modified as:
\vspace{-3pt}
\begin{equation}
\hat{\epsilon} = \epsilon_\theta(\btau^i, \varnothing, i) + \omega(\epsilon_\theta(\btau^i, \boldsymbol{y}, i) - \epsilon_\theta(\btau^i, \varnothing, i)),
\label{eq:hat_epsilon}
% \vspace{-2pt}
\end{equation}
where $\omega$ controls the guidance strength, and $\varnothing$ denotes the absence of conditioning, the part equal to unconditional diffusion learned from Eq.~\ref{eq:loss_uncond}. The training objective becomes:
\vspace{-5pt}
\begin{equation}
\mathcal{L}_{\mathit{free}}(\theta) = \mathbb{E}_{i, \btau, \epsilon}\left[\left|\epsilon - \epsilon_\theta\left(\btau^i, (1 - \beta) \boldsymbol{y}(\btau^i) + \beta \varnothing, i\right)\right|^2\right].
\label{eq:loss_diff}
\end{equation}
% where $\beta$ controls the condition dropout rate to balance sample diversity and context adherence. 
During sampling, trajectories are generated with the modified noise $\hat{\epsilon}$, employing re-parameterization technique.
% by iteratively applying the noise prediction model 

\subsection{Classifier-guided Conditional Policy}
\label{sec:c-guided formulation}
While classifier-free diffusion offers a streamlined approach, its conditioning flexibility relies solely on implicit representations within the training data. 
% This becomes particularly restrictive when adapting to novel task variations that, while related to the training scenarios, require novel goal specification. 
Classifier-guided approach, in contrast, enables direct reward or goal conditioning through gradient-based guidance.
% To formulate it, we re-write the conditional diffusion process:
% \vspace{-5pt}
% \begin{equation}
% \label{eq:diff_plan}
% q(\btau^{i} | \btau^{i-1}), \;\;\;\; p_{\theta}(\btau^{i-1}|\btau^{i}, \boldsymbol{y}(\btau)),
% \vspace{-2pt}
% \end{equation}
% where $\boldsymbol{y}(\btau)$ encodes trajectory-specific information such as return $\mathcal{J}(\btau^0)$ or constraints. 

% The optimization objective becomes:
% \vspace{-3pt}
% \begin{equation}
% \theta^*=\arg \min_\theta-\mathbb{E}{\btau^0}\left[\log p\theta(\btau^{0} | \boldsymbol{y}(\btau^0))\right]
% \label{eq:cond_gen_model}
% \end{equation}

For reward maximization, we introduce trajectory optimality $\mathcal{O}_{t}$ at timestep $t$, following a Bernoulli distribution where ${p(\mathcal{O}_t=1) = \exp (\gamma^{t} \mathcal{R}(\bs_t, \ba_t))}$. The diffusion process can be naturally extended to incorporate conditioning by sampling from perturbed distributions: 
\vspace{-6pt}
\begin{equation}
\label{eq:perturbed}
\tilde{p}_\theta(\btau{}) = p(\btau{} \mid \mathcal{O}_{1:T}=1) \propto p_{\theta}(\btau{}) p(\mathcal{O}_{1:T}=1 \mid \btau{})
\vspace{-3pt}
\end{equation}

Under Lipschitz conditions on $p(\mathcal{O}_{1:T} \mid \btau^{i})$~\cite{feller2015theory}, the reverse diffusion process follows:
\vspace{-6pt}
\begin{equation}
\label{eq:guided}
p_\theta(\btau^{i-1} \mid \btau^{i}, \mathcal{O}_{1:T}) \approx \mathcal{N}(\btau^{i-1}; \mu_{\theta} + \alpha\Sigma g, \Sigma),
\vspace{-3pt}
\end{equation}
where the guidance gradient $g$ is:
\vspace{-6pt}
\begin{equation}
\begin{aligned}
g &= \nabla_{\btau} \log p(\mathcal{O}_{1:T} \mid \btau) |_{\btau = \mu_{\theta}} \\
\vspace{-2pt}
&= \sum_{t=0}^{T} \gamma^{t} \nabla_{\bs_t,\ba_t} \mathcal{R}(\bs_t, \ba_t) |_{(\bs_t,\ba_t)=\mu_t}
= \nabla_{\btau} \mathcal{J}(\mu_{\theta}).
\end{aligned}
\vspace{-8pt}
\end{equation}

For goal-conditioned tasks, the constraint can be simplified by directly substituting conditional values at each diffusion timestep $i \in \{0, 1, ..., N\}$.


==> sec/table/main.tex <==
\begin{table*}
\centering
\small
\resizebox{0.8\textwidth}{!}{
    \begin{tabular}{lccc|lccc}
    \toprule
          & \textbf{20} & \textbf{50} & \textbf{100} & & \textbf{20} & \textbf{50} & \textbf{100} \\
    \midrule
    \textbf{\textit{Apple Cabinet Storage}} & & & & \textbf{\textit{Block Hammer Beat}} & & & \\
    DP &  &  & \cellcolor{gray!15} & DP &  &  & \cellcolor{gray!15}0.0±0.0 \\
    DP3 (XYZ) &  &  & \cellcolor{gray!15} & DP3 (XYZ) &  & 57.0±11.5 & \cellcolor{gray!15}52.7±4.0  \\
    DP3 (XYZ+RGB) &  &  & \cellcolor{gray!15} & DP3 (XYZ+RGB) &  &  & \cellcolor{gray!15} \\
    \midrule
    \textbf{\textit{Block Handover}} & & & & \textbf{\textit{Block Sweep}} & & & \\
    DP &  & 3.0±3.5 & \cellcolor{gray!15}8.7±3.2 & DP &  &  & \cellcolor{gray!15} \\
    DP3 (XYZ) &  & \cellcolor{gray!15}86.0±9.5 & 69.0±12.3 & DP3 (XYZ) &  &  & \cellcolor{gray!15} \\
    DP3 (XYZ+RGB) &  &  & \cellcolor{gray!15} & DP3 (XYZ+RGB) &  &  & \cellcolor{gray!15} \\
    \midrule
    \textbf{\textit{Blocks Stack (Easy)}} & & & & \textbf{\textit{Blocks Stack (Hard)}} & & & \\
    DP &  & 0.0±0.0 & \cellcolor{gray!15}2.3±1.5 & DP &  & 0.0±0.0 & \cellcolor{gray!15}0.3±0.6 \\
    DP3 (XYZ) & / & / & / & DP3 (XYZ) & / & / & / \\
    DP3 (XYZ+RGB) &  &  & \cellcolor{gray!15} & DP3 (XYZ+RGB) &  &  & \cellcolor{gray!15} \\
    \midrule
    \textbf{\textit{Container Place}} & & & & \textbf{\textit{Diverse Bottles Pick}} & & & \\
    DP &  & 11.7±8.0 & \cellcolor{gray!15}27.7±6.4 & DP &  & 1.3±0.6 & \cellcolor{gray!15}8.7±3.2 \\
    DP3 (XYZ) &  & 77.0±2.0 & \cellcolor{gray!15}86.3±2.5 & DP3 (XYZ) &  & 39.3±3.8 & \cellcolor{gray!15}39.3±9.6 \\
    DP3 (XYZ+RGB) &  &  & \cellcolor{gray!15}70.3+-3.2 & DP3 (XYZ+RGB) &  &  & \cellcolor{gray!15} \\
    \midrule
    \textbf{\textit{Dual Bottles Pick (Easy)}} & & & & \textbf{\textit{Dual Bottles Pick (Hard)}} & & & \\
    DP &  & 34.7±7.6 & \cellcolor{gray!15}88.3±2.1 & DP &  & 34.3±6.0 & \cellcolor{gray!15}54.7±4.0 \\
    DP3 (XYZ) &  & 71.7±7.0 & \cellcolor{gray!15}48.2±13.8 & DP3 (XYZ) &  & 48.0±4.6 & \cellcolor{gray!15}60.3±5.5 \\
    DP3 (XYZ+RGB) &  &  & \cellcolor{gray!15}67.7+-22.7 & DP3 (XYZ+RGB) &  &  & \cellcolor{gray!15}58.7±4.2 \\
    \midrule
    \textbf{\textit{Empty Cup Place}} & & & & \textbf{\textit{Mug Hanging}} & & & \\
    DP &  & 32.3±6.7 & \cellcolor{gray!15}77.3±20.2 & DP &  & 0.0±0.0 & \cellcolor{gray!15}0.0±0.0 \\
    DP3 (XYZ) &  & 74.7±5.8 & \cellcolor{gray!15}79.7±12.1 & DP3 (XYZ) &  & 9.3±3.1 & \cellcolor{gray!15}12.3±1.2 \\
    DP3 (XYZ+RGB) &  &  & \cellcolor{gray!15} & DP3 (XYZ+RGB) &  &  & \cellcolor{gray!15} \\
    \midrule
    \textbf{\textit{Pick Apple Messy}} & & & & \textbf{\textit{Shoe Place}} & & & \\
    DP &  & 7.3±1.2 & \cellcolor{gray!15}7.0±3.0 & DP &  & 10.3±5.1 & \cellcolor{gray!15}29.7±11.8 \\
    DP3 (XYZ) &  & 8.7±3.2 & \cellcolor{gray!15}16.0±3.0 & DP3 (XYZ) &  &  & \cellcolor{gray!15}54.0±6.9 \\
    DP3 (XYZ+RGB) &  &  & \cellcolor{gray!15} & DP3 (XYZ+RGB) &  &  & \cellcolor{gray!15}58.0±3.0 \\
    \midrule
    \textbf{\textit{Shoes Place}} & & & & \textbf{\textit{Average}} & & & \\
    DP &  & 0.7±0.6 & \cellcolor{gray!15}2.3±1.2 & DP &  &  & \cellcolor{gray!15} \\
    DP3 (XYZ) &  &  & \cellcolor{gray!15}13.0±1.7 & DP3 (XYZ)  &  &  & \cellcolor{gray!15} \\
    DP3 (XYZ+RGB) &  &  & \cellcolor{gray!15} & DP3 (XYZ+RGB) &  &  & \cellcolor{gray!15} \\
    \bottomrule
    \end{tabular}}
\end{table*}
